Sibyl: Understanding and Addressing the Usability Challenges of Machine Learning In High-Stakes Decision Making

Machine learning (ML) is being applied to a diverse and ever-growing set of domains. In many cases, domain experts - who often have no expertise in ML or data science - are asked to use ML predictions to make high-stakes decisions. Multiple ML usability challenges can appear as result, such as lack of user trust in the model, inability to reconcile human-ML disagreement, and ethical concerns about oversimplification of complex problems to a single algorithm output. In this paper, we investigate the ML usability challenges that present in the domain of child welfare screening through a series of collaborations with child welfare screeners. Following the iterative design process between the ML scientists, visualization researchers, and domain experts (child screeners), we first identified four key ML challenges and honed in on one promising explainable ML technique to address them (local factor contributions). Then we implemented and evaluated our visual analytics tool, Sibyl, to increase the interpretability and interactivity of local factor contributions. The effectiveness of our tool is demonstrated by two formal user studies with 12 non-expert participants and 13 expert participants respectively. Valuable feedback was collected, from which we composed a list of design implications as a useful guideline for researchers who aim to develop an interpretable and interactive visualization tool for ML prediction models deployed for child welfare screeners and other similar domain experts.

==> Figures/experiment_diagram.tex <==
\usetikzlibrary{shapes.geometric, arrows}
\usetikzlibrary{calc}

\tikzstyle{exp} = [rectangle, thick, minimum width=3cm, minimum height=1cm,text centered, draw=black, text width=6cm, fill=green!20, font=\bfseries]
\tikzstyle{rq} = [rectangle, minimum width=4cm, minimum height=1cm,text centered, draw=black, text width=8cm, fill=blue!20]
\tikzstyle{vis} = [rectangle, minimum width=3cm, minimum height=1cm,text centered, draw=black, text width=6cm, fill=yellow!20, font=\bfseries]
\tikzstyle{not_inc} = [rectangle, minimum width=3cm, minimum height=1cm,text centered, draw=black, text width=6cm, fill=gray!20, font=\bfseries]
\tikzstyle{arrow} = [thick,->,>=stealth]

\begin{figure}
    \centering
    \scalebox{.75}{%
    \begin{tikzpicture}[node distance=2cm]
    \node (trust) [exp] {Pilot Study 1: Trust};
    \node (usefulness) [exp, below of=trust] {Pilot Study 2: Usefulness};
    \node (accuracy) [exp, below of=usefulness] {Pilot Study 3: Accuracy};
    \node (outcome) [exp, below of=accuracy] {Simulation Study: Outcome};
    \node (field) [not_inc, below of=outcome] {Field Study};
    
    
    \node (r1) [rq, right of=trust, xshift=7cm, yshift=0cm] {R.1 Improving the quality of call screener decisions};
    \node (r2) [rq, below of=r1] {R.2 Increasing the rate with which call screeners consider the model score in decision making};
    \node (r3) [rq, below of=r2] {R.3 Increasing the rate with which call screeners recognize cases where the model may be inaccurate};
    \node (r4) [rq, below of=r3] {R.4 Developing an explanation pipeline specifically geared for the chosen domain};
    \node (r5) [rq, below of=r4] {R.5 Deploying a machine learning explanation tool in the domain};
    
    \node (details) [vis, right of=r1, xshift=7cm, yshift=2cm] {Feature Contributions};
    \node (changes) [vis, below of=details] {Custom Feature Changes};
    \node (swaps) [vis, below of=changes] {Universal Feature Changes};
    \node (nn) [vis, below of=swaps] {Nearest Neighbor - features};
    \node (nn_outcome) [vis, below of=nn] {Nearest Neighbor - outcomes};
    \node (importance) [vis, below of=nn_outcome] {Global Feature Importance};
    \node (dist) [vis, below of=importance] {Feature Distributions};
    
    \draw [arrow] (trust.east) -- (r1.west);
    \draw [arrow] (trust.east) -- (r2.west);
    \draw [arrow] (trust.east) -- (r4.west);
    \draw [arrow] (trust.east) -- (r5.west);
    
    \draw [arrow] (usefulness.east) -- (r1.west);
    \draw [arrow] (usefulness.east) -- (r2.west);
    \draw [arrow] (usefulness.east) -- (r4.west);
    \draw [arrow] (trust.east) -- (r5.west);
    
    \draw [arrow] (accuracy.east) -- (r1.west);
    \draw [arrow] (accuracy.east) -- (r3.west);
    \draw [arrow] (accuracy.east) -- (r5.west);
    
    \draw [arrow] (outcome.east) -- (r1.west);
    \draw [arrow] (outcome.east) -- (r4.west);
    \draw [arrow] (outcome.east) -- (r5.west);
    
    \draw [arrow] (field.east) -- (r1.west);
    \draw [arrow] (field.east) -- (r5.west);
    
    \draw[arrow] (r1.east) -- (details.west);
    \draw[arrow] (r1.east) -- (changes.west);
    \draw[arrow] (r1.east) -- (swaps.west);
    \draw[arrow] (r1.east) -- (nn.west);
    \draw[arrow] (r1.east) -- (nn_outcome.west);
    \draw[arrow] (r1.east) -- (importance.west);
    \draw[arrow] (r1.east) -- (dist.west);
    
    \draw[arrow] (r2.east) -- (details.west);
    \draw[arrow] (r2.east) -- (changes.west);
    \draw[arrow] (r2.east) -- (swaps.west);
    \draw[arrow] (r2.east) -- (nn.west);
    \draw[arrow] (r2.east) -- (nn_outcome.west);
    \draw[arrow] (r2.east) -- (importance.west);
    \draw[arrow] (r2.east) -- (dist.west);
    
    \draw[arrow] (r3.east) -- (details.west);
    \draw[arrow] (r3.east) -- (changes.west);
    \draw[arrow] (r3.east) -- (swaps.west);
    \draw[arrow] (r3.east) -- (nn.west);
    \draw[arrow] (r3.east) -- (nn_outcome.west);
    
    \draw[arrow] (r4.east) -- (details.west);
    \draw[arrow] (r4.east) -- (changes.west);
    \draw[arrow] (r4.east) -- (swaps.west);
    \draw[arrow] (r4.east) -- (nn.west);
    \draw[arrow] (r4.east) -- (nn_outcome.west);
    \draw[arrow] (r4.east) -- (importance.west);
    \draw[arrow] (r4.east) -- (dist.west);
    
    \draw[arrow] (r5.east) -- (details.west);
    \draw[arrow] (r5.east) -- (changes.west);
    \draw[arrow] (r5.east) -- (swaps.west);
    \draw[arrow] (r5.east) -- (nn.west);
    \draw[arrow] (r5.east) -- (nn_outcome.west);
    \draw[arrow] (r5.east) -- (importance.west);
    \draw[arrow] (r5.east) -- (dist.west);


    \end{tikzpicture}
    }
    \caption{Project summary.}
    \label{fig:experiments}
\end{figure}

==> Figures/pilot_study_diagram.tex <==
\usetikzlibrary{shapes.geometric, arrows}
\usetikzlibrary{calc}

\tikzstyle{study_start} = [rectangle, thick, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black, text width=6cm, fill=blue!20, font=\bfseries]
\tikzstyle{study_step} = [rectangle, minimum width=3cm, minimum height=1cm,text centered, draw=black, text width=6cm, fill=orange!30]
\tikzstyle{record} = [rectangle, minimum width=3cm, minimum height=1cm,text centered, draw=black, text width=6cm, fill=green!30]
\tikzstyle{calc} = [rectangle, rounded corners, thick, minimum width=3cm, minimum height=1cm,text centered, draw=black, text width=8cm, fill=red!30, font=\bfseries]
\tikzstyle{metric} = [rectangle, rounded corners, thick, minimum width=3cm, minimum height=1cm,text centered, draw=black, text width=4cm, fill=red!30]
\tikzstyle{arrow} = [thick,->,>=stealth]

\begin{figure}
    \centering
    \scalebox{.55}{%
    \begin{tikzpicture}[node distance=2cm]
    \node (start) [study_start, inner sep=0cm] {Pilot Study 1: Usability and Usefulness};
    \node (intro) [study_step, below of=start] {Show users details about case and model prediction};
    \node (explanation) [study_step, below of=intro] {Show users explanations through \Sibyl{}};
    \node (explanation_monitor) [record, below of=explanation] {Monitor explanation use};
    \node (screen) [study_step, below of=explanation_monitor] {Ask for screening decision};
    \node (reflection) [record, below of=screen] {Ask reflection questions about usefulness and trust};
    \node (calc) [calc, below of=reflection] {Calculate and parse metrics};
    \node (calc_time) [metric, below of=calc] {Time spent on each explanation type};
    \node (calc_freq) [metric, left of=calc_time, xshift=-3cm] {Frequency of use of each tool interaction};
    \node (calc_helpful) [metric, right of=calc_time, xshift=3cm] {Subjective helpfulness of each explanation type};
    \node (calc_ui) [metric, left of=calc_freq, xshift=-3cm] {Difficult or confusing elements of UI};
    \node (calc_trust) [metric, right of=calc_helpful, xshift=3cm] {Trust in model and influences to trust};
    
    
    \draw [arrow] (start) -- (intro);
    \draw [arrow] (intro) -- (explanation);
    \draw [arrow] (explanation) -- (explanation_monitor);
    \draw [arrow] (explanation_monitor) -- (screen);
    \draw [arrow] (screen) -- (reflection);
    \draw [arrow] (reflection) -- (calc);
    \draw [arrow] (calc) -- (calc_time);
    \draw [arrow] (calc) -- (calc_freq);
    \draw [arrow] (calc) -- (calc_helpful);
    \draw [arrow] (calc) -- (calc_ui);
    \draw [arrow] (calc) -- (calc_trust);
    
    \end{tikzpicture}
    }

    \caption{Usefulness user study.}
    \label{fig:pilot}
\end{figure}

==> Figures/user_studies.tex <==
\usetikzlibrary{shapes.geometric, arrows}
\usetikzlibrary{calc}

\tikzstyle{study_start} = [rectangle, thick, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black, text width=6cm, fill=blue!20, font=\bfseries]
\tikzstyle{study_step} = [rectangle, minimum width=3cm, minimum height=1cm,text centered, draw=black, text width=6cm, fill=orange!30]
\tikzstyle{record} = [rectangle, minimum width=3cm, minimum height=1cm,text centered, draw=black, text width=6cm, fill=green!30]
\tikzstyle{calc} = [rectangle, rounded corners, thick, minimum width=3cm, minimum height=1cm,text centered, draw=black, text width=8cm, fill=red!30, font=\bfseries]
\tikzstyle{arrow} = [thick,->,>=stealth]

\begin{figure}
    \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \scalebox{.55}{%
    \begin{tikzpicture}[node distance=2cm]
    \node (start) [study_start, inner sep=0cm] {Pilot Study 1: Trust};
    \node (intro) [study_step, below of=start] {Show users details about case};
    \node (model) [study_step, below of=intro] {Show users model prediction};
    \node (explanation) [study_step, below of=model, xshift=3.5cm, yshift=-1cm] {Show users explanations};
    \node (explanation_monitor) [record, below of=explanation] {Monitor explanation use};
    \node (no_explanation) [study_step, below of=model, xshift=-3.5cm, yshift=-1cm] {No further information};
    \node (screen) [study_step, below of=explanation_monitor, xshift=-3.5cm] {Ask for screening decision};
    \node (record) [record, below of=screen] {Record screening decision};
    \node (calc) [calc, below of=record] {Compare similarity between screening decision and model prediction, with and without explanation};
    
    \draw [arrow] (start) -- (intro);
    \draw [arrow] (intro) -- (model);
    \draw [arrow] (model) node[anchor=east, yshift=-1.5cm, xshift=-2cm] {Control condition}-- (no_explanation);
    \draw [arrow] (model) node[anchor=west, yshift=-1.5cm, xshift=2cm] {Experimental condition}-- (explanation);
    \draw [arrow] (explanation) -- (explanation_monitor);
    \draw [arrow] (explanation_monitor) -- (screen);
    \draw [arrow] (no_explanation) -- (screen);
    \draw [arrow] (screen) -- (record);
    \draw [arrow] (record) -- (calc);
    
    \end{tikzpicture}
    }
    \caption{Trust user study.}
    \label{fig:trust}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
    \centering
    \scalebox{.55}{%
    \begin{tikzpicture}[node distance=2cm]
    \node (start) [study_start, inner sep=0cm] {Pilot Study 3: Usefulness};
    \node (intro) [study_step, below of=start] {Show users details about case};
    \node (model) [study_step, below of=intro] {Show users model prediction};
    \node (explanation) [study_step, below of=model] {Show users explanations, with limitations on how many explanations they may use};
    \node (explanation_monitor) [record, below of=explanation] {Monitor explanation use};
    \node (screen) [study_step, below of=explanation_monitor] {Ask for screening decision};
    \node (calc) [calc, below of=screen] {Calculate time spent using each explanation type};
    
    \draw [arrow] (start) -- (intro);
    \draw [arrow] (intro) -- (model);
    \draw [arrow] (model) -- (explanation);
    \draw [arrow] (explanation) -- (explanation_monitor);
    \draw [arrow] (explanation_monitor) -- (screen);
    \draw [arrow] (screen) -- (calc);
    
    \end{tikzpicture}
    }

    \caption{Usefulness user study.}
    \label{fig:useful}
\end{subfigure}
\end{figure}


==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> Tables/context_factors_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[ht]
\footnotesize
\begin{tabular}{{p{0.2\textwidth}p{0.3\textwidth}p{0.20\textwidth}p{0.15\textwidth}}}

\toprule
\textbf{Context Factors}              & \textbf{Categorizations}                                               & \textbf{Example domain}          & \textbf{Main Usability Concerns} \\ \midrule
\multirow{4}{*}{Degree of Automation} & Fully autonomous, human not involved in decision making                & Level 5 self-driving car \cite{} & None                             \\
                                      & Machine makes decisions, human monitors                                & Level 4 self-driving car \cite{} & \DS, \CN, \AC, \ET            \\
                                      & Machine suggests decisions, humans make decisions                      & Violation flagging programs      & \TR, \DS, \CN, \AC, \ET           \\
                                      & \textbf{Machine provides auxiliary information, humans makes decisions} & Child welfare screening         & \TR, \DS, \CT, \UT, \ET           \\ \midrule
\multirow{4}{*}{Decision time}        & Immediate                                                              & Level 5 self-driving car         & None                             \\
                                      & Seconds                                                                & Aircraft emergency response      & \CN, \ET                        \\
                                      & \textbf{Minutes}                                                       & Child welfare screening          & \TR, \DS, \CN, \ET                     \\
                                      & Hours                                                                  & Non-emergency medical procedures & \TR, \DS, \CN, \ET                     \\ \midrule
Human technical expertise             & Little to none                                                         & Child welfare                    & \TR, \CT, \UT                                 \\
                                      & Experience with data science                                           & Finance                          &                                  \\
                                      & Machine learning/Data science expert                                   & Meta-learning models             & \TR                                 \\ \midrule
Human domain expertise                & Little to none                                                         & Autonomous aircraft (to passengers)              & \CN                              \\
                                      & Basic understanding/Intuition                                          & Crowdsourcing                    & \CN                              \\
                                      & Domain expert                                                          & Child welfare screening          & \TR, \DS, \AC                     \\ \midrule
Associated Risk                       & Low                                                                    & Camera roll image sorting        &                                  \\
                                      & Medium                                                                 & Mail sorting                     &                                  \\
                                      & High                                                                   & Emergency medical procedures     &                                  \\ \bottomrule
\end{tabular}
\caption{Domain context factors that may influence the usability of an ML model. The right-most column references the codes introduced in table \ref{tab:usability_concerns}. Note that in this table, we only discuss the usability concerns present when using the model is already being used for active decision making. }
\label{tab:context_factors_table}
\end{table}

==> Tables/interfaces_grid.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[t]
\caption[The proposed \Sibyl{} \pages{}, and the challenges they were theorized to address.]{The proposed \Sibyl{} \pages{} (left column), the challenges they were theorized to address (middle column, using the codes from Table \ref{tab:usability_concerns}), and the reasons we expected these \pages{} to address the given challenges (right column). \TR: Lack of trust in the model. \DS: Difficulty reconciling disagreements. \CT: Confusing prediction target. \ET: Ethical concerns.}
\begin{tabular}{x{0.25\linewidth}P{0.04\linewidth}P{0.04\linewidth}P{0.04\linewidth}P{0.04\linewidth}p{.50\linewidth}}
\toprule
\multirow{2}{*}{\textbf{Interface}}       & \textbf{Challenges Addressed}  & \multirow{2}{*}{\textbf{How does it address the challenge?}}                                              \\
& \TR{} & \DS{} & \CT{} & \ET{} & \\
\midrule
Case-Specific Details    & \TR                            & Reveals relevancy of considered factors                              \\
                         & \DS                            & Highlights factors that may have been missed or misused              \\
                         & \CT                            & Translates score to a concrete factor list                           \\
                         & \ET                            & Allows for critical thinking about factors and score                 \\ \midrule
Sandbox                  & \DS                            & Allows users to test theorized justifications                        \\
                         & \ET                            & Allows for thinking through what-if scenarios                        \\ \midrule
Similar Cases            & \TR                            & Provides information on past performance                             \\
                         & \ET                            & Provides a deeper look into the nuance of cases                      \\ \midrule
Global Factor Importance & \TR                            & Reveals how the model generally makes predictions                    \\
                         & \CT                            & Translates the score to a concrete factor list                       \\ \midrule
Factor Distributions     & \TR                            & Shows how well the model performed on past cases                     \\
                         & \CT                            & Shows the relationship between the risk score and removals from home \\ \bottomrule
\end{tabular}
\label{tab:interfaces}
\end{table*}

==> Tables/model_table.tex <==
\begin{table}[h]
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
\textbf{Model Name}                                     & \textbf{County} & \textbf{Output}                  & \textbf{Prediction Target}                 & \textbf{Current state} \\ \midrule
AFST \cite{vaithianathanDevelopingPredictiveModels2017} & Allegheny, PA   & \multirow{3}{*}{1-20 risk score} & \multirow{3}{*}{Removal in next two years} & Deployment             \\
DCDA \cite{vaithianathanImplementingChildWelfare2019}   & Douglas, CO     &                                  &                                            & Live testing           \\
LDAT                                                    & Larimer, CO     &                                  &                                            & Live testing           \\ \bottomrule
\end{tabular}
\caption{The PRM tools currently in use. This paper focuses on augmenting the LDAT.}
\label{tab:models}
\end{table}


==> Tables/needs_table.tex <==
\begin{table}[t]
\centering
\begin{tabularx}{\linewidth}{@{} >{\raggedright\arraybackslash}p{0.25\linewidth} l  >{\raggedright\arraybackslash}p{0.15\linewidth}  >{\raggedright\arraybackslash}p{0.15\linewidth} >{\raggedright\arraybackslash}X@{}}
\toprule
\textbf{Need} & \textbf{Design Goals} & \textbf{Method} & \textbf{Sibyl Screen}  & \textbf{Caveats} \\ \midrule
Understand what information led to the score & G1, G2, G3 & SHAP & Details, Feature Importance    & Machine learning models must be presented in an understandable way \\\\[-1.5ex]
Understand how the model gets the score from the information given & G1   & Natural Language Explanation & Feature Importance & Should not be overly technical \\\\[-1.5ex]
Be able to investigate ``what-if'' style explanations   & G2, G3 & Counterfactuals & Sandbox& May cause screeners to interpret model as having causal meaning    \\\\[-1.5ex]
See how the model predicted on past, familiar cases & G1, G3 & Nearest neighbors, dataset summary & Similar Cases, Feature Distributions & May encourage making decisions based on comparisons to past cases  \\ 
\bottomrule
\end{tabularx}%
\caption{The explanation needs of the child welfare screeners, as given during initial interviews. Each \Sibyl{} screen was designed to meet a need that was expressed in interviews or inferred based on behavior during the use-case simulation. Meeting each need also comes with certain caveats that we must be aware of when developing explanations.}
\label{tab:needs}
\end{table}

==> Tables/needs_table_2.tex <==
\begin{table}[t]
\centering
\begin{tabularx}{\linewidth}{@{} >{\raggedright\arraybackslash}p{0.25\linewidth}  >{\raggedright\arraybackslash}p{0.15\linewidth}  >{\raggedright\arraybackslash}p{0.15\linewidth} >{\raggedright\arraybackslash}X@{}}
\toprule
\textbf{Interview Request} & \textbf{Method} & \textbf{Sibyl Screen}  & \textbf{Caveats} \\ \midrule
Understand what information led to the score & SHAP & Details, Feature Importance    & Machine learning models must be presented in an understandable way \\\\[-1.5ex]
Understand how the model gets the score from the information given  & Natural Language Explanation & Feature Importance & Should not be overly technical \\\\[-1.5ex]
Be able to investigate ``what-if'' style explanations   & Counterfactuals & Sandbox& May cause screeners to interpret model as having causal meaning    \\\\[-1.5ex]
See how the model predicted on past, familiar cases  & Nearest neighbors, dataset summary & Similar Cases, Feature Distributions & May encourage making decisions based on comparisons to past cases  \\ 
\bottomrule
\end{tabularx}%
\caption{The explanation needs of the child welfare screeners, as given during initial interviews. Each \Sibyl{} screen was designed to meet a need that was expressed in interviews or inferred based on behavior during the use-case simulation. Meeting each need also comes with certain caveats that we must be aware of when developing explanations.}
\label{tab:needs}
\end{table}

==> Tables/trust_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[t]
\footnotesize
\begin{tabular}{{p{0.35\textwidth}p{0.06\textwidth}p{0.50\textwidth}}}
\toprule
Category                                                                                                                      & \begin{tabular}[c]{@{}l@{}}\# of \\ answers\end{tabular} & Sample answers                                                                                                                                                                                                                 \\ \midrule
\begin{tabular}[c]{@{}l@{}}General comments about being shown \\ protective and risk factors (Details page)\end{tabular}      & 8                                                        & \begin{tabular}[c]{@{}l@{}}``The details and the risk and protective factors and the \\ contribution they have'', ``Info in the details and risk factors''\end{tabular}                                                            \\
\begin{tabular}[c]{@{}l@{}}Specific factors listed as risk or \\ protective (Details page)\end{tabular}                       & 8                                                        & \begin{tabular}[c]{@{}l@{}}``The past number of child welfare involvements (listed in the \\ features listed)'', ``The risk factors involved, especially prior \\ placements, benefits, and current CPS involvement''\end{tabular} \\
The number of factors listed                                                                                                  & 5                                                        & ``Very few risk factors'', ``The lack of protective factors''                                                                                                                                                                      \\
Score agreed with screener intuition                                                                                      & 10                                                       & \begin{tabular}[c]{@{}l@{}}``... the children are not residing with the alleged perpetrators \\ which I would assume would reduce the risk score'', \\ ``Model prediction makes sense''\end{tabular}                               \\
Explanation agreed with screener intuition                                                                                & 3                                                        & ``Risk factors made sense for the model prediction number''                                                                                                                                                                      \\
General comments about sandbox page                                                                                           & 1                                                        & ``Details under sandbox of why the risk level was so high''                                                                                                                                                                      \\
\begin{tabular}[c]{@{}l@{}}General comments about the explanation\\  providing more information or understanding\end{tabular} & 6                                                        & ``Allowed for more understanding'', ``History clarification''                                                                                                                                                                      \\ \bottomrule
\end{tabular}
\caption{Summary of reasons expert participants listed for having ``a great deal'', ``a lot'' or ``a moderate amount'' of trust in the model. The second and third columns refer to participant answers to the question ``What made you trust the model more?''}
\label{tab:trust_increase}
\end{table*}

\begin{table*}[t]
\footnotesize
\begin{tabular}{{p{0.35\textwidth}p{0.06\textwidth}p{0.50\textwidth}}}
\toprule
Category & \begin{tabular}[c]{@{}l@{}}\# of \\ answers\end{tabular} & Sample answers                                                                                               \\ \midrule
A specific, key factor was not considered by the model & 3                                                       & ``This is a case for law enforcement, not CPS'', ``... it may have been handled during the open case"           \\
The importance weighting of factors was off            & 2                                                       & ``Young, vulnerable children being left alone is still cause for concern, despite past involvement''           \\ 
The score disagreed with screener intuition            & 3                                                       & ``Seems high, no {[}health history{]}, no real proof of any drug use, no proof child is at any risk of abuse'' \\
There was some confusion about information presented   & 2                                                       & ``There were discrepancies between the info in the referral and the info provided by the tool''                \\
The screener wanted more information                   & 2                                                       & ``I would want to see other referrals for the family''  
 \\ \bottomrule
\end{tabular}
\caption{Summary of reasons expert participants listed for having ``a little'', ``not at all'' trust in the model. The second and third columns refer to participant answers to the question ``What made you trust the model more?''}
\label{tab:trust_decrease}
\end{table*}

==> Tables/trust_table_updated.tex <==
\begin{table*}[t]
\caption{Summary of answers to the question ``what made you trust the model more/less'' among expert participants who listed having ``\textit{a great deal}'', ``\textit{a lot}'' or ``\textit{a moderate amount}'' of trust in the model. The first column lists the general themes we found in the answers. The second column list the number of answers that fell within each theme. The final column lists selected answers for each theme.}
\footnotesize
\begin{tabular}{{p{0.4\textwidth}p{0.06\textwidth}p{0.44\textwidth}}}
\toprule
Category                                                                                                                      & \begin{tabular}[c]{@{}l@{}}\# of \\ answers\end{tabular} & Sample answers                                                                                                                                                                                                                 \\ \midrule
General comments about being shown protective and risk factors (Details page)      & 8                                                        & ``\textit{The details and the risk and protective factors and the contribution they have}'' ``\textit{Info in the details and risk factors}''                                                            \\
Specific factors listed as risk or protective (Details page)                    & 8                                                        & ``\textit{The past number of child welfare involvements (listed in the features listed)}'', ``\textit{The risk factors involved, especially prior placements, benefits, and current CPS involvement}'' \\
The number of factors listed (Details page)                                                                                                  & 5                                                        & ``\textit{Very few risk factors}'', ``\textit{The lack of protective factors}''                                                                                                                                                                      \\
The score agreed with screener intuition                                                                                      & 10                                                       & ``\textit{...the children are not residing with the alleged perpetrators which I would assume would reduce the risk score}'',  ``\textit{Model prediction makes sense}''                             \\
The explanation agreed with screener intuition                                                                                & 3                                                        & ``\textit{Risk factors made sense for the model prediction number}''                                                                                                                                                                      \\
General comments about sandbox page                                                                                           & 1                                                        & ``\textit{Details under sandbox of why the risk level was so high}''                                                                                                                                                                      \\
General comments about the explanation providing more information or understanding & 6                                                        & ``\textit{Allowed for more understanding}'', ``\textit{History clarification}''                                                                                                                                                                      \\ \bottomrule
\end{tabular}
\label{tab:trust_increase}
\end{table*}

\begin{table*}[ht!]
\caption{Summary of answers to the question ``what made you trust the model more/less'' among expert participants who listed having ``\textit{a little}'' or ``\textit{not at all}'' trust in the model. The first column lists the general themes we found in the answers. The second column list the number of answers that fell within each theme. The final column lists selected answers for each theme.}
\footnotesize
\begin{tabular}{{p{0.4\textwidth}p{0.06\textwidth}p{0.44\textwidth}}}
\toprule
Category & \begin{tabular}[c]{@{}l@{}}\# of \\ answers\end{tabular} & Sample answers                                                                                               \\ \midrule
A specific, key factor was not considered by the model & 3                                                       & ``\textit{This is a case for law enforcement, not CPS}'', ``\textit{...it may have been handled during the open case}''           \\
The importance weighting of factors was off (Details page)            & 2                                                       & ``\textit{Young, vulnerable children being left alone is still cause for concern, despite past involvement}''           \\ 
The score disagreed with screener intuition            & 3                                                       & ``\textit{Seems high, no health history, no real proof of any drug use, no proof child is at any risk of abuse}'' \\
There was some confusion about information presented   & 2                                                       & ``\textit{There were discrepancies between the info in the referral and the info provided by the tool}''                \\
The screener wanted more information                   & 2                                                       & ``\textit{I would want to see other referrals for the family}''  
 \\ \bottomrule
\end{tabular}
\label{tab:trust_decrease}
\end{table*}

==> Tables/user_study_questions.tex <==
\begin{table*}[t]
\caption{Questions asked in the UI/UX and Outcome Evaluation user studies.}
\centering
\begin{tabular}{{p{0.15\textwidth}p{0.2\textwidth}p{0.55\textwidth}}}
\toprule                                                    
\textbf{When?}                   & \textbf{Response Type}   & \textbf{Question}                                                 \\ \midrule
Beginning                        & Multiple choice          & What is your experience with child welfare screening?             \\ \midrule
\multirow{7}{*}{After each case} & Multiple choice          & Would you choose to screen-in or screen-out?                      \\
                                 & 5-point Likert scale     & How confident are you in your decision?                           \\
                                 & 5-point Likert scale     & How much did the prediction score impact your decision?           \\
                                 & 5-point Likert scale     & How much did you trust the model’s prediction for this case?      \\
                                 & Free response            & What caused you to trust the model more or less?                  \\
                                 & Multiple-multiple choice & What explanations, if any, did you find helpful?                  \\
                                 & Free response            & Any other comments?                                               \\ \midrule
\multirow{4}{*}{End}             & 5-point Likert scale     & How helpful did you find the model's predictions overall?         \\
                                 & 5-point Likert scale     & How helpful did you find the Sibyl tool's explanations?           \\
                                 & Multiple-multiple choice & Which explanation did you find most helpful overall?              \\
                                 & Free response            & Were there any feature categories you found more or less helpful? \\ \bottomrule
\end{tabular}
\label{tab:questions_asked}
\end{table*}

==> Tables/user_study_table.tex <==
\begin{table}[h]
\small
\centering
\begin{tabularx}{\linewidth}{@{}r| X p{0.1\linewidth}p{0.15\linewidth}@{}}
% \toprule
\hline\\[-2ex]
\textbf{User Study} & \textbf{Objectives} & \textbf{Data Used} & \textbf{Participant Pool}  \\[0.5ex] 
% \midrule
\hline\\[-2ex]
UI/UX & 
\begin{minipage}[t]{\linewidth}
\begin{itemize}[nosep,leftmargin=*,after=\strut,label={--}]
\item Evaluating explanation usefulness and usability 
\item Adjusting interface to be more user-friendly 
\item Determining which explanations to use for active decision making  
\end{itemize}
\end{minipage} \par
& Synthetic & 
General populace, Domain experts 
\\%&&&\\[-1.5ex]
Outcome Evaluation & 
\begin{minipage}[t]{\linewidth}
\begin{itemize}[nosep,leftmargin=*,after=\strut,label={--}]
\item Quantifying change in decision making resulting from tool 
\end{itemize}
\end{minipage} \par
& Historic & 
Domain experts 
\\%&&&\\[-1.5ex]
Live Testing & 
\begin{minipage}[t]{\linewidth}
\begin{itemize}[nosep,leftmargin=*,after=\strut,label={--}]
\item Quantifying change in decision making resulting from tool 
\item Observing effect of tool in real context 
\end{itemize}
\end{minipage}
& Current cases & 
Domain experts (active screeners)   
% \\ \bottomrule
\\[1ex] 
\hline
\end{tabularx}
\smallskip
\caption{Summary of user studies needed to deploy \Sibyl{}. The first study listed was run for this paper.}
\label{tab:user_studies}
\end{table}

\iffalse
\begin{table}
\small
\begin{tabular}{@{}llllll@{}}
\toprule
                               & Participants         & Metric     & Task               & Information Given                                                                                & Information Gathered                                                    \\ \midrule
\multirow{3}{*}{Pilot Studies} & \multirow{3}{*}{Any} & Trust      & Make Decision      & \begin{tabular}[c]{@{}l@{}}Case information,\\ model prediction, \\ one explanation\end{tabular} & \begin{tabular}[c]{@{}l@{}}Decisions made, \\ time taken\end{tabular}   \\
                               &                      & Accuracy   & Guess Model Output & \begin{tabular}[c]{@{}l@{}}Case information,\\ one explanation\end{tabular}                      & \begin{tabular}[c]{@{}l@{}}Predictions made, \\ time taken\end{tabular} \\
                               &                      & Usefulness & Make Decision      & \begin{tabular}[c]{@{}l@{}}Case information,\\ model prediction,\\ all explanations\end{tabular} &  Explanations used                                                                          \\ \midrule
Simulation Studies             &                      &            &                    &                                                                                                  &                                                                         \\ \midrule
Live Studies                   &                      &            &                    &                                                                                                  &                                                                         \\ \bottomrule
\end{tabular}
\caption{Summary of user studies.}
\label{tab:studies}
\end{table}
\fi

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

